Convex block-sparse linear regression with expanders -- provably

Sparse matrices are favorable objects in machine learning and optimization. When such matrices are used, in place of dense ones, the overall complexity requirements in optimization can be significantly reduced in practice, both in terms of space and run-time. Prompted by this observation, we study a convex optimization scheme for block-sparse recovery from linear measurements. To obtain linear sketches, we use expander matrices, i.e., sparse matrices containing only few non-zeros per column. Hitherto, to the best of our knowledge, such algorithmic solutions have been only studied from a non-convex perspective. Our aim here is to theoretically characterize the performance of convex approaches under such setting. Our key novelty is the expression of the recovery error in terms of the model-based norm, while assuring that solution lives in the model. To achieve this, we show that sparse model-based matrices satisfy a group version of the null-space property. Our experimental findings on synthetic and real applications support our claims for faster recovery in the convex setting -- as opposed to using dense sensing matrices, while showing a competitive recovery performance.

==> algorithms.tex <==
\section{Algorithms for solving \eqref{}}

==> experiments_prev.tex <==
\section{Experiments}{\label{sec:experiments}}

\subsection{Performance evaluation}

Synthetic examples. 
\begin{itemize}
	\item [$(i)$] Show how $\ell_{2,1}$-norm minimization helps over $\ell_1$-norm minimization. High dimensional case - the highest we can such that we can do 50 Monte-Carlo iterations in reasonable amount of time. In the same plot, $x$-axis is the number of measurements and $y$-axis is the recovery rate. The experiments should be repeated many times (e.g., 50 Monte-Carlo iterations). We can show both mean and median cases. Also mention the time needed for both algorithms (probably $\ell_1$-norm is much faster but we hope we can reconstruct cases with much less number of samples - tradeoff). Other alternative is to create a phase transition plot but this would need much more experiments.
	\item [$(ii)$] Focus on $\ell_{2,1}$-norm minimization. Here we compare Gaussian, Bernoulli and Sparse matrices (i don't know whether we should compare with other matrices). Same experiment as above but now we compare different sensing matrices. We should also give examples where dense matrices lead to slow execution time (put a time-wall that $\ell_{2,1}$-norm minimization needs a lot of time).
\end{itemize}

\begin{figure}[!ht]
	\begin{center}
		\includegraphics[width=0.45\textwidth]{figs/Compl1_l21_expanders_gaussian} \hspace{-0.5cm}
		\includegraphics[width=0.45\textwidth]{figs/Compl1_l21_expanders_binary}
	\end{center}
	%\caption{Median error per iteration of factored gradient descent algorithm for different step sizes, over 20 Monte Carlo iterations. The number of measurements is fixed to $C_{\text{sam}} \cdot n \cdot r$ for varying $C_{\text{sam}} \in \left\{4, 6, 10 \right\}$. Here, $n = 1204$ and rank $r = 5$. Curves show convergence behavior of Algorithm \ref{algo:altgrad} as a function of the step size selection. Οne can observe that arbitary step size selections can lead to slow convergence. Moreover, good constant step size selections -- for a specific problem configuration, do not necessarily translate into good performance for a different setting; \text{e.g.}, observe how the constant step size convergence rates worsen \textit{faster}, as we decrease the number of observations.}{\label{exp_fig:00}}
\end{figure}

\begin{figure}[!ht]
	\begin{center}
		\includegraphics[width=0.9\textwidth]{figs/Compl21_expanders_gaussian_recovery}
	\end{center}
%	\caption{Median error per iteration of factored gradient descent algorithm for different step sizes, over 20 Monte Carlo iterations. The number of measurements is fixed to $C_{\text{sam}} \cdot n \cdot r$ for varying $C_{\text{sam}} \in \left\{4, 6, 10 \right\}$. Here, $n = 1204$ and rank $r = 5$. Curves show convergence behavior of Algorithm \ref{algo:altgrad} as a function of the step size selection. Οne can observe that arbitary step size selections can lead to slow convergence. Moreover, good constant step size selections -- for a specific problem configuration, do not necessarily translate into good performance for a different setting; \text{e.g.}, observe how the constant step size convergence rates worsen \textit{faster}, as we decrease the number of observations.}{\label{exp_fig:01}}
\end{figure}

\subsection{Structured covariance estimation}

We consider the problem of estimating a \emph{structured} sparse covariance from sketches of sample vectors \cite{dasarathy2013sketching}. Let $\Z = \left\{Z_1, Z_2, \dots, Z_{\sqrt{\dim}}\right\}$ be a $\sqrt{\dim}$-dimensional variable vector that follows the zero mean Gaussian distribution with \emph{unknown} covariance $\boldsymbol{\Sigma}$, i.e., $\Z \sim \mathcal{N}\left(\mathbf{0}, \boldsymbol{\Sigma}\right)$. Assume that we have access to this model only through a collection of samples $\left\{\z_i\right\}_{i = 1}^{q}$, drawn independently and identically distributed according to $\mathcal{N}(\mathbf{0}, \boldsymbol{\Sigma})$.

In many cases of interest, the unknown $\boldsymbol{\Sigma}$ has structure; in particular, we assume that $\boldsymbol{\Sigma}$ is group sparse, i.e., variables are sparsely correlated. One way to estimate $\boldsymbol{\Sigma}$ is through sample paths of the statistical process. That is, we repeatedly sample the source until we statistically acquire enough information to recover the unknown sparse correlations. However, in the high-dimensional setting, one needs to \emph{store} the collection of samples $\left\{\z_i\right\}_{i = 1}^{q}$, which might be prohibitive when $\dim$ and $q$ is large. 

To this end, it may be desirable to reduce the dimensionality $\sqrt{\dim}$ by \emph{pooling covariates together}. That is, we sketch samples $\z_i$ with expander matrix $\widehat{\Ph} \in \left\{0, 1\right\}^{\sqrt{\numsam} \times \sqrt{\dim}}$ such that we only observe:
\begin{align*}
\w_i = \widehat{\Ph} \z_i \in \R^{\sqrt{\numsam}}, \quad i = 1, \dots, q,
\end{align*} with $\sqrt{\numsam} \ll \sqrt{\dim}$. 
Observe that, since $\widehat{\Ph}$ is a binary matrix, each entry of $\w_i$ ``accumulates'' a random selection of variables from $\Z$. This way we create sketches of variables $\Z$.

Note that the empirical covariance of $\left\{ \w_i\right\}_{i = 1}^q$ satisfies:
\begin{align*}
\widehat{\boldsymbol{\Sigma}}_{\w} &= \frac{1}{q} \sum_{i = 1}^q \w_i \w_i^\top \nonumber \\ &= \widehat{\Ph} \left(\frac{1}{q} \sum_{i = 1}^q \z_i \z_i^\top\right) \widehat{\Ph}^\top \nonumber \\ &= \widehat{\Ph} \widehat{\boldsymbol{\Sigma}}_{\z} \widehat{\Ph}^\top,
\end{align*} where $\widehat{\boldsymbol{\Sigma}}_{\z} = \frac{1}{q} \sum_{i = 1}^q \z_i \z_i^\top$ is the empirical covariance of the original samples $\{\z_i\}_{i = 1}^q$. For the rest of our discussion, we assume $q$ is large enough such that $\widehat{\boldsymbol{\Sigma}}_{\z}$ is a good approximation to $\boldsymbol{\Sigma}$, i.e., we can recover the unknown sparsity pattern of $\boldsymbol{\Sigma}$ from the approximate $\widehat{\boldsymbol{\Sigma}}_{\z}$.

Using the Kronecker product property:
\begin{align*}
\A \X \mathbf{B}^\top \stackrel{\text{vectorize}}{\Longleftrightarrow} \left(\mathbf{B} \otimes \A\right) \cdot \text{vec}(\X),
\end{align*} we can rewrite our observation model as a sparse recovery problem:
\begin{align*}
\obs := \text{vec}(\widehat{\boldsymbol{\Sigma}}_{\w}) = \underbrace{\left(\widehat{\Ph} \otimes \widehat{\Ph}\right)}_{:= \Ph} \underbrace{\text{vec}(\widehat{\boldsymbol{\Sigma}}_{\z})}_{:= \x^\star},
\end{align*} where $\obs \in \R^{\numsam}$, $\x^\star \in \R^\dim$ is the group-sparse structured unknown vector and $\Ph \in \{0,1\}^{\numsam \times \dim}$ is an expander matrix according to the following definition.

\begin{definition}[Tensor graphs \cite{dasarathy2013sketching}]
Let a graph $\left(\sqrt{\dim}, \sqrt{\numsam}, \EE \right)$ be a bipartite graph with $\sqrt{\dim}$ left (variable) nodes, $\sqrt{\numsam}$ right (check) nodes and a set of edges $\EE$ with adjacency matrix $\widehat{\Ph} \in \{0, 1\}^{\sqrt{\numsam} \times \sqrt{\dim}}$. We define the tensor graph $\left(\dim, \numsam, \EE \otimes \EE \right)$ with adjacency matrix $\Ph = \widehat{\Ph} \otimes \widehat{\Ph} \in \{0, 1\}^{\numsam \times \dim}$ such that such that $\{(i, i'),~(j, j')\} \in \EE \otimes \EE$ if and only if $\{i, j\} \in \EE$.
\end{definition}

\begin{figure}[!tb]
	\begin{center}
		\includegraphics[width=0.4\columnwidth]{figs/vectorize}
	\end{center}
	\caption{Toy example for vectorization of structured sparse covariates into non-overlapping group sparse vector.}{\label{sec_exp:fig1}}
\end{figure}

The above suggest that we can use the tools presented in this work to recover the sparsity pattern of the covariance matrix. 

Some comments on the above:

\begin{itemize}
\item [$(i)$] I know that the solution should be positive definite (also symmetric), but we can just leave it as it is and show that we can do well without these constraints in practice.
\item [$(ii)$] I believe the experiment should go as follows: fix the group sparsity over the covariates of the unknown $\boldsymbol{\Sigma}$, draw samples from the Gaussian distribution, create a sketch expander $\Ph$ and observe the sketched observations $\w_i$. Then, we use the Kronecker product tool and use $\ell_{2,1}$-minimization to do find out which group of covariates is on. 
\item [$(iii)$] We are not interested in the statistical point of view of the experiment: someone can say that we might not have enough samples such that $\widehat{\boldsymbol{\Sigma}}_{\z}$ is a good approximation of $\boldsymbol{\Sigma}$. This is out of the scope of the paper.
\end{itemize}
